A New Approach to Fair Distribution of Welfare

We consider transferable-utility profit-sharing games that arise from settings in which agents need to jointly choose one of several alternatives, and may use transfers to redistribute the welfare generated by the chosen alternative. One such setting is the Shared-Rental problem, in which students jointly rent an apartment and need to decide which bedroom to allocate to each student, depending on the student's preferences. Many solution concepts have been proposed for such settings, ranging from mechanisms without transfers, such as Random Priority and the Eating mechanism, to mechanisms with transfers, such as envy free solutions, the Shapley value, and the Kalai-Smorodinsky bargaining solution. We seek a solution concept that satisfies three natural properties, concerning efficiency, fairness and decomposition. We observe that every solution concept known (to us) fails to satisfy at least one of the three properties. We present a new solution concept, designed so as to satisfy the three properties. A certain submodularity condition (which holds in interesting special cases such as the Shared-Rental setting) implies both existence and uniqueness of our solution concept.

==> solutionConcepts.tex <==
\section{Comparison to some prior solution concepts}
\label{appendix:bargaining}

Many bargaining solutions have been suggested in the past. Below we discuss some of the most known ones, and show that none of them satisfy all the properties we consider desirable.
The solutions we discuss include the Nash bargaining solution and the Kalai-Smorodinsky bargaining solution. %, the Shapley value and  the Nucleolus.
As transfers are allowed, each of them picks a division of the utility generated by the social maximizing outcome among the players. These solutions can be defined to dominate RP, but need not lie in the upper core. This last fact has the following undesirable consequences.

The Nash bargaining solution is not reasonable from above ($u_i \le W_{max}(i)$ might fail for some agent $i$), and
it fails to satisfy even the weak decomposition property.

The Kalai-Smorodinsky bargaining solution is  reasonable from above, % ($u_i \le W_{max}(i)$ for each agent $i$),
but it fails to satisfy even the weak decomposition property.

Below we also discuss another solution concept, the nucleolus. A version of it that lies in the upper core can be defined in a natural way, but it need not dominate the disagreement utilities.
%TO DO:

%Nash requires Independence of irrelevant alternatives (IIR), while KS does not.




\subsection{The Nash bargaining solution}

The Nash bargaining solution, when applied in our setting, becomes identical to the egalitarian solution, equalizing the gains of all agents above their respective disagreement utilities.   As such, it dominates RP, but need not lie it the upper core. Moreover, the Nash bargaining solution need not be reasonable from above.  Namely, it may hold that $u_i > W_{max}(i)$ for some agent $i$. The following example illustrates this point.


Consider a setting with two agents and a two alternatives. The first agent has values of $24$ and $0$ for the two alternatives, while the second agents has value of $0$ and $4$.   Random priority will give the agents expected utilities of $12$ and $2$, respectively.  These are the disagreement utilities, and their total is only $14$, which is $10$ less than the maximum welfare of $24$.  The Nash bargaining solution will give each of them an additional utility of $5$ so the final utilities will be $17$ and $7$.  In particular, the utility of the second agent is higher than the utility offered to her by the best alternative.


Likewise, the Nash bargaining solution fails to satisfy the even the weak decomposition property. The example in Appendix \ref{sec:KS} can serve to illustrate this last point (details omitted).



% Consider the example in Section \ref{sec:KS}. The Nash Bargaining solution will equalize the amount each agent gets from the extra amount of 8 that needs to be divided among the agents beyond the disagreement utilities. Thus, each will get additional utility of $2$, and the final utilities will be $8,10,8$ and $14$. The first two agents together get $18$ instead of $16$ (the maximal they could get in any alternative), and the last two agents get $22$ instead of $24$. This means that there is a transfer between the two components, not satisfying the weak decomposition property (or the group upper bound for the first two agents).




\subsection{The Kalai-Smorodinsky bargaining solution}
\label{sec:KS}

The Kalai-Smorodinsky (KS) solution has the following geometric interpretation.
Each alternative corresponds to a point in $\Re_+^n$, specifying the utility of each of the  $n$ agents.
The \emph{point of best utilities} is the point with coordinate for each agent equal to the best utility she gets in any feasible alternative.
The Kalai-Smorodinsky solution is the intersection of the Pareto frontier with the line from the disagreement point to the point of best utilities.

We note that while our solution aims to equalize utility gains (compared to disagreement utilities) as much as possible (subject to upper core constraints), the KS solution aims to equalize the fraction of the utility improvements (from the disagreement to the best point).


Like in our solution, the KS solution never gives any agent more than her utility in the best alternative for her.
Yet, the KS solution might fail to satisfy the upper core constraints for groups of more than one player.
Consequently, it fails to satisfy even the weak decomposition property. This is illustrated by the following example:

Consider an item allocation setting in which there are four agents and four items, and in each alternative each agent receives one item. Hence there are $4! = 24$ possible alternatives. The valuation of each agent for each item is presented  in the following table:

\begin{tabular}{|c|c|c|c|c|}
	\hline
	% after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
	Example & {\bf Item 1} & {\bf Item 2} & {\bf Item 3} & {\bf Item 4} \\
	\hline
	{\bf Agent 1} & 4 & 8 & 0 & 0 \\
	{\bf Agent 2} & 4 & 12 & 0 & 0 \\
	{\bf Agent 3} & 0 & 0 & 4 & 8 \\
	{\bf Agent 4} & 0 & 0 & 4 & 20 \\
	\hline
\end{tabular}

The problem decomposes to the first two agents (with maximum welfare $16$) and last two agents (with maximum welfare $24$), giving a total maximum welfare $40$. Random priority will give the agents expected utilities of $6, 8, 6$ and $12$, respectively.
These are the disagreement utilities, and their total is only $32$, which is $8$ less than the maximum welfare.

The best utility each of the agents can get is $8, 12, 8$ and  $20$, respectively, for a total of $48$.
Subtracting the disagreement values this gives the agents $2, 4, 2$ and  $8$, respectively, which in total is $16$ above the disagreement point,
rather than $8$ that can be divided among the agents.


The KS solution lowers what each agent gets (above disagreement) in a uniform rate, meaning that the agents will get utilities $7, 10, 7$ and $16$, respectively. That is, each agent gets half the gap between his disagreement utility and his best utility.
Hence the first two agents together get $17$ instead of $16$ (the maximal they could get in any alternative), and the last two agents get $23$ instead of $24$. This means that there is a transfer between the two components, not satisfying the weak decomposition property (or the group upper bound for the first two agents).


\subsection{The Nucleolus}

Once we introduce the WS-core, the concept of {\em nucleolus}~\cite{Schmeidler69} can be adapted to our setting for the purpose of selecting a solution within the WS-core. For the purpose of defining the nucleolus, one needs to describe the setting as a coalitional game, where there is a characteristic function associated with sets of agents. Given our notion of upper core and the fact that we have a profit game (in which agents share the welfare increase that results from selecting a maximum welfare alternative), it is most natural to use $D(S) = W_{max}({\cal{N}}) - W_{max}({\cal{N}} \setminus S)$ as a characteristic function (see the end of Section~\ref{sec:uppercore}). Applying the nucleolus framework to this characteristic function is then equivalent to selecting a solution that satisfies the upper core constraints with as large a margin as possible (measured in terms of a lexicographic vector of the margins). This solution satisfies the weak decomposability property (because it is in the upper core, see Proposition~\ref{pro:upperdecomposes}), but need not satisfy the domination constraints (and hence might not be in the WS-core). Even in the room (item) allocation setting (which is submodular), there are examples in which the nucleolus fails to dominate the Random Priority mechanism. The instance described in Appendix~\ref{app:RP} serves as one such example (for the same reason that it shows that the Shapley value solution does not dominate RP -- see the last paragraph of the proof of Proposition~\ref{prop:Shapley-prop-app} for an explanation). To enforce the Nucleolus solution to lie within the WS-core, one may modify it so that it selects a solution that satisfies the upper core constraints with as large a margin as possible, subject to satisfying the domination constraints. In contrast, our \lexmaxws\ solution satisfies the domination constraints with as large a margin as possible, subject to the upper core constraints. Whereas having a large margin for the domination constraints has a clear purpose (giving agents incentives to give up the reference point and adapt our mechanism), we do not see as useful a purpose for keeping a large margin from the upper core constraints. Moreover, modification of the nucleolus concept so as to satisfy the domination constraints causes it lose some features that make the (unmodified) nucleolus an attractive solution concept, such as consistency for reduced games~\cite{MPT92}.




==> water-filling-proof.tex <==
\subsection{The water filling algorithm}\label{app:water}
In this section we prove Proposition \ref{pro:water}: when the $W_{max}$ is submodular, the water filling algorithm computes the \lexmax\ solution.

\begin{proof}
By design, the water filling algorithm satisfies all domination constraints and all constraints of the anticore. Likewise, it produces a lexicographically maximal solution subject to these constraints. It remains to show that by the end of the algorithm, the anticore constraint $\sum_{i\in {\cal{N}}} u(i) \le W_{max}({\cal{N}})$ is tight (meaning that all welfare has been shared by the agents), where here $u(i)=\sum_{t=1}^{j} x_j$ is the utility of agent $i$ that was locked right after iteration $j$ %at the end of the algorithm
(and $u(S)$ will serve as shorthand notation for $\sum_{i\in S} u_i$).

When the water filling algorithm ends, every agent is involved in a tight anticore constraint. Suppose for the sake of contradiction that the constraint $u({\cal{N}}) \le W_{max}({\cal{N}})$ is not tight. Let $S_j$ (for $j = 1, 2, \ldots$) be the sets of agents whose constraints became tight in iteration $j$ of
the execution of the water filling algorithm.
Consider a set function $W'_{max}$ that is identical to $W_{max}$, except that $W'_{max}({\cal{N}}) = u({\cal{N}}) < W_{max}({\cal{N}})$. Then $W'_{max}$ is submodular, all the sets $S_j$ referred to above are tight with respect to it, and so is $\cal{N}$. By Lemma~\ref{lem:lattice}, all unions of these sets $S_j$ are also tight with respect to $W'_{max}$. By repeatedly taking unions, we arrive at two sets $S$ and $T$ such that $S \cup T = {\cal{N}}$, both $u(S) = W'_{max}(S) = W_{max}(S)$ and $u(T) = W'_{max}(T) = W_{max}(T)$ hold, and $u(S \cap T) = W'_{max}(S\cap T) < W_{max}(S\cap T)$. By linearity, $u({\cal{N}}) = u(S) + u(T) - u(S \cap T) \ge W_{max}(S) + W_{max}(T) - W_{max}(S\cap T)$. By submodularity of $W_{max}$ we have that $W_{max}({\cal{N}}) \le W_{max}(S) + W_{max}(T) - W_{max}(S\cap T)$. These last two inequalities contradict our assumption that $u({\cal{N}}) < W_{max}({\cal{N}})$.
\end{proof}

When $W_{max}$ is not submodular, the water filling algorithm might fail to find the \lexmax\ solution, even when the WS-core is nonempty. Consider an instance with three agents and three alternatives, with the following valuation functions.

\begin{tabular}{|c|c|c|c|}
  \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
   & {\bf Alternative 1} & {\bf Alternative 2} & {\bf Alternative 3} \\
\hline
  {\bf Agent 1} & 0 & -2 & 2 \\
  {\bf Agent 2} & 0 & 2 & -1 \\
  {\bf Agent 3} & 0 & 2 & -1 \\
  \hline
\end{tabular}

When Alternative~1 serves as the disagreement alternative, the WS-core is nonempty and contains a unique solution, given by choosing Alternative~2 (that has total welfare of~2), and transfers such that the utility of Agent~1 is~0 and of the other two agents is~1. Being unique, this is also the \lexmax\ solution.  However, the water filling algorithm will start by giving evert agent a utility of $\frac{1}{2}$. At this point every agent is part of a tight anticore constraint), and the algorithm ends before distributing all the welfare to the agents.



